A-optimal encoding weights for nonlinear inverse problems, with applications to the Helmholtz inverse problem

The computational cost of solving an inverse problem governed by PDEs, using multiple experiments, increases linearly with the number of experiments. A recently proposed method to decrease this cost uses only a small number of random linear combinations of all experiments for solving the inverse problem. This approach applies to inverse problems where the PDE solution depends linearly on the right-hand side function that models the experiment. As this method is stochastic in essence, the quality of the obtained reconstructions can vary, in particular when only a small number of combinations are used. We develop a Bayesian formulation for the definition and computation of encoding weights that lead to a parameter reconstruction with the least uncertainty. We call these weights A-optimal encoding weights. Our framework applies to inverse problems where the governing PDE is nonlinear with respect to the inversion parameter field. We formulate the problem in infinite dimensions and follow the optimize-then-discretize approach, devoting special attention to the discretization and the choice of numerical methods in order to achieve a computational cost that is independent of the parameter discretization. We elaborate our method for a Helmholtz inverse problem, and derive the adjoint-based expressions for the gradient of the objective function of the optimization problem for finding the A-optimal encoding weights. The proposed method is potentially attractive for real-time monitoring applications, where one can invest the effort to compute optimal weights offline, to later solve an inverse problem repeatedly, over time, at a fraction of the initial cost.

==> abstract.tex <==
We introduce a method to systematically select among random encoding weights,
for inverse problem with multiple right-hand sides, when these weights are
sampled from the uniform spherical distribution. Drawing from recent
developments in optimal experimental design for infinite-dimensional Bayesian
inverse problems, we introduce two Bayesian formulations of this weight
selection problem. In addition, we rigorously formulate a bilevel
Hessian-constrained optimization problem for the computation of weights that
optimally verify our selection criterion. 



==> method_r26194.tex <==
\section{Methodology to select from random encoding weights with uniform
spherical distribution}
\label{sec:form}

Combining the results from section~\ref{sec:infdimB} with elements from optimal
experimental design, we introduce a rigorous method to select encoding weights
from a family of samples, all drawn from the uniform spherical distribution.
In particular, we define two alternate expressions for the objective functional
$\obj(\ww)$ that governs this selection process.

In the Bayesian framework, the posterior covariance quantifies the uncertainty
in the reconstruction.  Since the posterior covariance depends on the weights
(see section~\ref{sec:postw}), we can select the weights that lead to a
reconstruction with the least uncertainty. 
In the field of optimal
experimental design, there are various design criteria that measure the
statistical quality of the reconstructed parameter~\cite{Pukelsheim93}.  
%
In the present work, we rely on the A-optimal design
criterion~\cite{Pukelsheim93,AtkinsonDonev92}, which aims to minimize the trace
of the posterior covariance, 
or equivalently, to minimize the average of the posterior variance.
That is, we favor the weights with the smallest trace of the
posterior covariance $\obj(\ww)=\text{tr}(\Cgeneric)$ with $\Cgeneric$ given by
$\Cgn$~\eqref{eq:cpostgnenc} or $\Clap$~\eqref{eq:cpostlaplaceenc}. 

An alternate view of the A-optimal design criterion is that of
minimizing the expected Bayes risk of the MAP estimator, which coincides with
the trace of the posterior covariance in the case of a linear inverse
problem~\cite{AlexanderianPetraStadlerEtAl14,ChalonerVerdinelli95,HaberHoreshTenorio08}.
This interpretation of
A-optimal criterion, for linear inverse problems, can be stated as the average
mean squared error between the MAP estimator (i.e., the parameter reconstruction) and the
true parameter (e.g., see~\cite{AlexanderianPetraStadlerEtAl14}). While this
interpretation of A-optimality is restricted to linear inverse problems, it
provides another motivation for our choice of the design criterion. In our
numerical results, we explore this relation between minimizing the trace of the
posterior covariance and the mean squared distance between the MAP point and the true
parameter. We observe in our numerical results that minimizing the trace of the
posterior covariance does result in smaller errors for the parameter
reconstruction.


\subsection{Dependence of the operators $\Cgn$ and $\Clap$ on $\ww$}
\label{sec:postw}

The dependence of the operators $\Cgn$~\eqref{eq:cpostgnenc} and
$\Clap$\eqref{eq:cpostlaplaceenc} on the weights is twofold.
First these operators depend on the encoded parameter-to-observable maps that
depend explicitly on the weights, $\pto(\ww^i;m) = \sum_{j=1}^{N_s} w_j^i
\pto_j(m)$.  Moreover, the posterior covariance operators also depend on the weights
through the MAP~point~(\ref{eq:infMAPenc}), which depends on the weights as
illustrated by~(\ref{eq:infMAPenc}) and~(\ref{eq:Jw}).

The dependence of 
the covariance operator $\Cgn$
on $\ww$ is straightforward to see.
In particular, 
using the chain-rule on the forward problem~$\mathcal{A}(m) u_i = f(\ww^i)$,
the Fr\'echet derivative of the
parameter-to-observable at the MAP~point is given by
%
\begin{equation} \label{eq:FF} 
\JJ_{\ww^i} = - B \mathcal{A}(m_\map(\ww))^{-1}
\frac{\partial \mathcal{A}(m) u_i}{\partial m} \Bigg|_{m = m_\map(\ww)} .
\end{equation}
%
Given $N_w$~encoded sources $\ww = (\ww^1, \ldots, \ww^{N_w})$ where $\ww^i \in
\R^{N_s}$, we emphasize the dependence of the posterior covariance on the
weights by writing $\Cgn = \Cgn(\ww)$.  The structure of the covariance
operator~$\Clap$ is more complicated. We detail the dependence of
$\Clap$ on $\ww$ for the application problem considered in the present paper in 
section~\ref{sec:wave}.  Note that in
the case of a linear parameter-to-observable map, both posterior
covariances~(\ref{eq:cpostgnenc}) and~(\ref{eq:cpostlaplaceenc}) are equal.


\subsubsection{Codomain of the encoding weights} 

In the present formulation the value of $\text{tr} \Big(
\mathcal{C}_\text{post}(\ww) \Big)$ scales with the norm of the
weights. For instance, applying a constant multiplicative factor~$\lambda>1$ to
all weights would reduce the influence of the prior in the computation of the
MAP point~(\ref{eq:infMAPenc}) for once. It would also inflate
the norm of the state variable~$u_i$ by that factor~$\lambda$, which would
then increase the size of the derivative~(\ref{eq:FF}).  
This would in turn artificially reduce the trace of
the posterior covariance~(\ref{eq:cpostgnenc}). A solution is to restrict the
codomain of the random encoding weights to a sphere of radius~$r$ in~$\R^{N_w
N_s}$ that we denote~$\SS_r$, i.e., 
$\SS_r \coloneqq \left\{ \ww \in \R^{N_w N_s}, \, | \ww | = r \right\}$; 
the uniform spherical distribution~$\Us(r)$ is an example of such distribution
and in the rest of that paper we assume the weights are sampled from that
distribution.  As discussed in section~\ref{sec:medparam}, the theory of random
source encoding dictates the use of~$r=\sqrt{N_w N_s}$. However this value is
arbitrary and can be compensated by an equivalent re-scaling of the
regularization parameter. Therefore for simplicity we use the value~$r=1$ in the
rest of that paper along with the notation~$\SS \coloneqq \SS_1$.

\subsection{Formulations of the weight selection process}
\label{sec:cplteformenc}

The selection of weights, from a family of randomly sampled encoding weights
$\ww \sim \Us(1)$, is governed by the criterion
%
\begin{equation*} 
\obj(\ww) = \text{tr}( \mathcal{C}_\text{post}(\ww) ). \end{equation*}
%
We introduced two alternatives for~$\mathcal{C}_\text{post}(\ww)$ in
section~\ref{sec:approxcov}. The Gauss-Newton formulation~$\obj_\mathup{GN}(\ww)$ is
based on the posterior covariance~(\ref{eq:cpostgnenc}),
%
\begin{equation} \label{eq:Wselgninf}
\obj_\mathup{GN}(\ww)  = \text{tr}(\HessGN^{-1}(\ww; m_\map(\ww)) ). 
\end{equation}
% 
While the Laplace formulation~$\obj_\mathup{L}(\ww)$ is based on the posterior
covariance~(\ref{eq:cpostlaplaceenc}),
\begin{equation} \label{eq:Wsellaplaceinf}
\obj_\mathup{L}(\ww) = \text{tr}(\Hess^{-1}(\ww; m_\map(\ww))).
\end{equation}

Note that both formulations require the
computation of the MAP~point which becomes computationally expensive for
large-scale problems.  Note also
that the Gauss-Newton Hessian is guaranteed to be positive definite everywhere
in (medium) parameter space, allowing fair comparisons of the
criterion~$\obj_\mathup{GN}$ at other locations than the MAP~point.  To avoid
the cost associated with the computation of the MAP~point, an additional simplification
of~\eqref{eq:Wselgninf} can be achieved  
by evaluating the posterior
covariance~(\ref{eq:cpostgnenc}) at a fixed reference parameter~$m_0$ chosen
appropriately,
%
\begin{equation} \label{eq:Wselgnlininf} \obj_0(\ww)  = \text{tr}(
\HessGN^{-1}(\ww; m_0)).  \end{equation}
%
This approximation sacrifices the dependence of the Fr\'echet derivative of the
parameter-to-observable map on the weights through the MAP~point~(\ref{eq:FF}).



\section{Formulations of the A-optimal encoding weights}
\label{sec:formweights}

The weight selection formulation introduced in section~\ref{sec:form}
provides a practical method to
objectively select the ``best'' encoding weights from an ensemble of weights
drawn from the uniform spherical distribution. 
%
As discussed in the introduction, an alternate approach to random source
encoding consists of 
developing a methodology to compute (deterministic) encoding weights, and that
is the focus of this section.
Using notations from section~\ref{sec:form},
we propose to compute the A-optimal encoding weights as the solution to the
constrained minimization problem
%
\[ \ww_c = \arg \min_{\ww \in \SS} \left\{ \obj(\ww) \right\} , \]
%
with $\Cgeneric$ given by $\Cgn$~\eqref{eq:cpostgnenc} or
$\Clap$~\eqref{eq:cpostlaplaceenc}. 
%
In that format, the A-optimal encoding weights can be interpreted as the weights
that minimize either the weight selection criterion~\eqref{eq:Wselgninf} or the
weight selection criterion~\eqref{eq:Wsellaplaceinf}.


However this highly nonlinear optimization problem requires the use of iterative
methods which involve repeated evaluations of the trace of the posterior
covariance.  Following discretization, the posterior covariance is a
high-dimensional  operator that is defined implicitly, i.e., through its
applications to vectors.  The exact computation of the trace of such operators,
and their derivatives with respect to encoding weights, is computationally
intractable.  For this reason, we propose an approximate formulation using a
randomized trace estimator (see~\cite{AvronToledo11,Hutchinson90} for the
theory, and~\cite{HaberDoelHoresh14,AlexanderianPetraStadlerEtAl14} for examples
of applications).


\paragraph{Infinite-dimensional trace estimation}
\label{sec:infdimtrestim}

Following the formulation in~\cite{AlexanderianPetraStadlerEtAl16}, let's
introduce the Gaussian measure~$\mu_\delta = \mathcal{N}(0, \mathcal{C}_\delta)$
where $\mathcal{C}_\delta = (I - \delta \Delta)^{-2}$.  Here $\Delta$ denotes
the Laplacian operator with homogeneous Neumann boundary conditions and $\delta
> 0$ a sufficiently small real number.  Then for any positive, self-adjoint and
trace-class operator~$\mathcal{K}$, we may use an estimator of form, 
%
\[ \text{tr}(\mathcal{K}) \approx \frac1{n_{tr}} \sum_{i=1}^{n_{tr}} \langle
\mathcal{K} z_i, z_i \rangle_\mathscr{H} , \] 
%
where the $z_i$ are drawn from~$\mu_\delta$.  In general, the number $n_{tr}$ of
trace estimator vectors depends on the spectral properties of $\mathcal{K}$. In
practice, for operators with clustered eigenvalues, reasonable approximations of
the trace can be obtained with a relatively small $n_{tr}$.

\paragraph{Formulations of the A-optimal encoding weights}
\label{sec:cplteform}
The optimization problem for finding A-optimal encoding weights is formulated as follows 
%
\begin{equation*} 
\min_{\ww \in \SS} \frac1{n_{tr}} \sum_{i=1}^{n_{tr}}
\langle \mathcal{C}_\text{post}(\ww) z_i, z_i \rangle.
\end{equation*}
%
Specializing to the cases of
$\obj_\mathup{GN}(\ww)$, based on the posterior
covariance~(\ref{eq:cpostgnenc}), and~$\obj_{\mathup{L}}(\ww)$, based on the posterior
covariance~(\ref{eq:cpostlaplaceenc}), respectively, results in the following 
formulations:
%
\begin{equation} \label{eq:Wcgninf}
\ww_c = \arg \min_{\ww \in \SS} \left\{ \frac1{n_{tr}} \sum_{i=1}^{n_{tr}}
\langle \HessGN^{-1}(\ww; m_\map(\ww)) z_i, z_i \rangle \right\},
\end{equation}
% 
\begin{equation} \label{eq:Wclaplaceinf}
\ww_c = \arg \min_{\ww \in \SS} \left\{ \frac1{n_{tr}} \sum_{i=1}^{n_{tr}}
\langle \Hess^{-1}(\ww; m_\map(\ww)) z_i, z_i \rangle \right\}.
\end{equation}
Again to avoid the cost associated with the computation of the
MAP~point, one can instead evaluate the Gauss-Newton Hessian in
formulation~\eqref{eq:Wcgninf} at a fixed reference parameter~$m_0$ chosen
appropriately; this leads to the following (simplified) optimization problem.
%
\begin{equation} \label{eq:Wcgnlininf} 
\ww_c = \arg \min_{\ww \in \SS} \left\{ \frac1{n_{tr}} \sum_{i=1}^{n_{tr}}
\langle \HessGN^{-1}(\ww; m_0) z_i, z_i \rangle \right\}.
\end{equation}
%
The formulation~\eqref{eq:Wcgnlininf} can be seen
as an extension of the formulation proposed in~\cite{HaberDoelHoresh14} with 
the underlying inverse problem formulated in function space, and being allowed
to be nonlinear.


